A computable analysis of variable words theorems

The Carlson-Simpson lemma is a combinatorial statement occurring in the proof of the Dual Ramsey theorem. Formulated in terms of variable words, it informally asserts that given any finite coloring of the strings, there is an infinite sequence with infinitely many variables such that for every valuation, some specific set of initial segments is homogeneous. Friedman, Simpson, and Montalban asked about its reverse mathematical strength. We study the computability-theoretic properties and the reverse mathematics of this statement, and relate it to the finite union theorem. In particular, we prove the Ordered Variable word for binary strings in ACA0.

==> parts/part4-fut-analysis.tex <==

Towsner~\cite{Towsner2012simple} gave a combinatorially simple proof of the Finite Union Theorem in $\aca^{+}$. He introduced the notion of full-match, and proved its existence over $\aca$ in~\cite[Lemma 2.7]{Towsner2012simple}.  However, the existence of a full-match is not known to be equivalent to $\aca$. This notion is the cornerstone of Towsner's proof, as having low${}_n$ full-matches for some fixed $n$ would be sufficient to obtain arithmetical solutions to the Finite Union Theorem. In this section, we improve the lower bound of the existence of a full-match by showing that it cannot be proven in $\wkl$.

\begin{definition}
Fix a coloring $c : \Pcal_{fin}(\Nb) \to r$.
Let $\Bcal \subseteq \Pcal_{fin}(\Nb)$ be a finite collection,
and let $\Ical \subseteq \Pcal_{fin}(\Nb) - \Bcal$ be an IP collection.
\begin{itemize}
	\item[(i)] $\Bcal$ \emph{left-matches} $\Ical$ if for every $S \in \Ical$, there is some $B \in \Bcal$ such that $c(B) = c(B \cup S)$. 
	\item[(ii)] $\Bcal$ \emph{right-matches} $\Ical$ if for every $S \in \Ical$, there is some $B \in \Bcal$ such that $c(S) = c(B \cup S)$. 
	\item[(iii)] $\Bcal$ \emph{full-matches} $\Ical$ if for every $S \in \Ical$, there is some $B \in \Bcal$ such that $c(B) = c(B \cup S) = c(S)$. 
\end{itemize}
\end{definition}

Note that in Towsner's paper~\cite{Towsner2012simple}, a right-match is called a half-match. A full-match is both a left-match and a right-match, but the converse is not true in general.

\begin{statement}
	$\lmfut_r$ denotes the statement ``For every coloring $c :\Pcal_{fin}(\Nb) \to r$, there is a finite collection $\Bcal \subseteq \Pcal_{fin}(\Nb)$  and an IP collection $\Ical \subseteq \Pcal_{fin}(\Nb) - \Bcal$ such that $\Bcal$ left-matches $\Ical$.
	The statements $\rmfut_r$ and $\rmfut_r$ are defined accordingly for the notions of right-match and full-match.
\end{statement}

Towsner~\cite[Lemma 2.5]{Towsner2012simple} proved $\rmfut_r$ over $\rca$. He also constructed in~\cite[Theorem 3.8]{Towsner2012simple} a computable instance of $\lmfut_2$ with no computable solution, therefore showing that $\rca \nvdash \lmfut_2$. We now adapt his proof to show that $\rca + \wkl \nvdash \lmfut_2$, by proving that $\lmfut_2$ implies the existence of hyperimmune functions.

The following theorem combines the techniques of Towsner~\cite[Theorem 3.8]{Towsner2012simple} and Csima and Mileti~\cite[Theorem 4.1]{Csima2009strength}. A familiarity with the mentioned proofs will simplify drastically the understanding of the proof of Theorem~\ref{thm:lmfut-opt}.



\begin{theorem}\label{thm:lmfut-opt}
There is a computable instance of $\lmfut_2$ such 
that every solution is of hyperimmune degree.
\end{theorem}
\begin{proof}
The strategy is the following: We will build a computable coloring $c : \Pcal_{fin}(\Nb) \to 2$ such that for every finite collection $\Bcal$ which left-matches an IP collection $\Ical$ we satisfy the following requirement for each $e \in \Nb$:
\begin{quote}
$\Rcal_e$: If $\Phi_e$ is total, then
there is an input $k_e$ such that 
$\Ical \cap [k_e, \Phi_e(k_e)] = \emptyset$.
\end{quote}
Here, $[a, b] = \{a, a+1, \dots, b \}$.
Suppose we have constructed $c$, and let $(\Bcal, \Ical)$ be such that $\Bcal$ left-matches~$\Ical$.
Let $p_\Ical$ be the $\Ical$-computable function which on input
$n$ searches for a set $S \in \Ical$ such that $\min S > n$ and outputs $\max S$. For every $e \in \Nb$, $p_\Ical(k_e) > \Phi_e(k_e)$.
Therefore $p_\Ical$ is not dominated by any computable function, hence is hyperimmune. We now explain how to build the coloring $c$.

Using a movable marker procedure, define for every $e \in \Nb$ and at every stage $s$ two inputs $x_{e,s}, y_{e,s} > e$ ordered as follows
$$
x_{0,s} < y_{0,s} < x_{1,s} < y_{1,s} < \dots 
$$
Moreover, if $\Phi_{e,s}(x_{e,s})\downarrow$, then $\Phi_{e,s}(x_{e,s}) < y_{e,s}$, and if $\Phi_{e,s}(y_{e,s})\downarrow$, then $\Phi_{e,s}(y_{e,s}) < x_{e+1,s}$. We can show by induction that each marker is moved at most finitely many times, and therefore $x_e = \lim_s x_{e,s}$ and $y_e = \lim_s y_{e,s}$ exist for every $e$. For every $e, s \in \Nb$, let $X_{e,s} = [x_{e,s}, \Phi_{e,s}(x_{e,s})]$ if $\Phi_{e,s}(x_{e,s})\downarrow$, and $X_{e,s} = \emptyset$ otherwise. The set $Y_{e,s}$ is defined accordingly.
	According to the previous observation, $X_e = \lim_s X_{e,s}$ and $Y_e = \lim_s Y_{e,s}$ exist for every $e \in \Nb$, and satisfy
$$
X_{0,s} < Y_{0,1} < X_{1,s} < Y_{1,s} < \dots
$$
The construction will work as follows. Using the combinatorics of Towsner~\cite[Theorem 3.8]{Towsner2012simple} (to be explained later), for every $e$, we will pick two sets $S \subseteq X_{e,s}$ and $T \subseteq Y_{e,s}$, and will ensure that $\{S, T, U\} \not \subseteq \Ical$ for every solution $(\Bcal, \Ical)$ to $c$, and cofinitely many finite sets $U$. If $\Phi_e$ is partial, our requirement is vacuously satisfied. If $\Phi_e$ is total, at some finite stage $t$, there will be some input $k_{S,T} \in \Nb$ such that $\Phi_{e,t}(k_{S,T})\downarrow$ and $\{S, T, U\} \not \subseteq \Ical$ for every $U \subseteq [k_{S,T}, \Phi_{e,t}(k_{S,T})]$. This way, we will have ensured that if $S$ and $T$ both belong to $\Ical$, then $\Ical \cap [k_{S,T}, \Phi_{e,t}(k_{S,T})] = \emptyset$. Since this is checked at a finite stage $t$, we then pick the next pair $S' \subseteq X_{e,t}$ and $T' \subseteq Y_{e,t}$ and do the same procedure, and so on until we have consumed all the pairs over $X_{e,t}$ and $Y_{e,t}$.
Therefore, we will have ensured that either $\Ical \cap X_e = \emptyset$, or $\Ical \cap Y_e = \emptyset$, or there is some $S \subseteq \Ical \cap X_e$ and $T \in \Ical \cap Y_e$
such that $\Ical \cap [k_{S,T}, \Phi_{e,t}(k_{S,T})] = \emptyset$. 

We say that a requirement $\Rcal_e$ is \emph{ready} at stage $s$ if 
$\Phi_{e,s}(x_{e,s})\downarrow$ and $\Phi_{e,s}(y_{e,s})\downarrow$.
Given a pair of finite sets $S^0 < S^1$, $\Rcal_e$ is \emph{$(S^0, S^1)$-satisfied for $\Rcal_e$} at stage $s$
if there is some $k > S^1$ such that $\Phi_{e,s}(k)\downarrow$
and for every set $A < S^0$, there is some $u < 2$ such that
for every $B \subseteq [k, \Phi_{e,s}(k)]$, $c(A) \neq c(A \cup S^u \cup B)$. In other words, $\Rcal_e$ is $(S^0,S^1)$-satisfied at stage $s$ if for every solution $(\Bcal, \Ical)$ to $c$ such that $S^0, S^1 \in \Ical$, $\Ical \cap [k, \Phi_{e,s}(k)] = \emptyset$. Note that a requirement may be ready at some stage, but not a later stage, whereas if $S^0 < S^1$ is satisfied for $\Rcal_e$ at some stage, then will always remain satisfied.
A requirement $\Rcal_e$ is \emph{satisfied} at stage $s$ if either $\Phi_e$ is partial, or it is $(S^0, S^1)$-satisfied for every pair $S^0 \subseteq X_{e,s}$ and $S^1 \subseteq Y_{e,s}$.

At any stage $s$ of the construction and for every $e < s$ such that $\Rcal_e$ is ready, we will have distinguished two sets $S^0_{e,s} \subseteq X_{e,s}$ and $S^1_{e,s} \subseteq Y_{e,s}$ which currently receive attention. They are chosen two be the least pair (in an arbitrary fixed order) which is not yet satisfied for $\Rcal_e$. The following two definitions are defined by Towsner~\cite[Theorem 3.8]{Towsner2012simple}.

A \emph{primary $s$-decomposition} of a set $B$, where $s = \max B$ is a tuple $i, u, Z, D$ such that $B = Z \cup S^u_{e,s} \cup D$, $Z < S^u_{e,s} < D$,
neither $Z$ nor $D$ contains $S^{1-u}_{i,s}$ as a subsequence, and there is no primary $s$-decomposition of $D$. Clearly, there is at most one primary $s$-decomposition of $B$.

We say that $B$ \emph{contains $e$ with polarity $v$} if there is a primary $\max B$-decomposition $i, u, Z, D$ of $B$ with either $e = i$ and $v = u$,
or $e$ contained in $Z$ with polarity $|v-u|$. Observe that whenever $B$ contains $e$, $B = Z \cup S^u_{e,t} \cup D$ for some $t \leq \max B$.

We now define our coloring by stages. At stage $s$, supposed we have already decided $c(B')$ whenever $\max B' < s$. Let $B$ be such that $\max B = s$. If $B$ has a primary $s$-decomposition $B = Z \cup S^u_{e,s} \cup D$, we set $c(B) = c(Z)$ if $u = 0$ and $c(B) \neq c(Z)$ if $u = 1$. If there is no primary $s$-decomposition of $B$, we set $c(B) = 0$. This completes the construction. We now turn to the verification.


\begin{claim}
For a total Turing functional $\Phi_e$, all $S \subseteq X_e$ and all $T \subseteq Y_e$, $\Rcal_e$ is $(S,T)$-satisfied at some stage. 
\end{claim}
\begin{proof}
Suppose not. Let $S \subseteq X_e$ and $T \subseteq Y_e$ be the least pair (in the previously fixed order) such that $\Rcal_e$ is not $(S,T)$-satisfied at any stage. Let $s$ be a stage such that for all $t \geq s$, $X_{e,t} = X_e$, $Y_{e,t} = Y_e$, and $\Rcal_e$ is $(S',T')$-satisfied for all the previous pairs $(S', T')$. By construction, $S^0_{e,t} = S$ and $S^1_{e,t} = T$.

It is easy to see that for any $B \geq s$, there is a $v_B$ such that
$A \cup S^u_e \cup B$ contains $e$ with polarity $|v_B - u|$ for all $A < \in \Bcal$. We now prove by induction on the length of $B$ that for all $B > s_1$ and $A < S^0_{e,t}$, $c(A \cup S^{v_B}_e \cup B) = c(A)$ and $c(A \cup S^{1-v_B}_e \cup B) \neq c(A)$. Given $u < 2$, let $D = A \cup S^u_e \cup B$. In particular, $D$ admits a primary $\max B$-decomposition $Z \cup S^{u'}_i \cup B'$. If we just have $e = i$, then $v_B = 0$ and the claim follows immediately from the decomposition of the coloring. Otherwise, we have two cases.
In the first case, $u' = 0$. Then $c(D) = c(Z)$ and $Z$ contains $e$ with polarity $|v_B - u|$. By induction hypothesis applied to $Z \setminus (A \cup S^u_e)$, $c(D) = c(Z) = c(A)$ if $u = v_B$ and $c(D) = c(Z) \neq c(A)$ if $u \neq v_B$. In the second case, $u' = 1$. Then $c(D) \neq c(Z)$ and $Z$ contains $e$ with polarity $1-|v_B-u|$. By induction hypothesis applied to $Z \setminus (A \cup S^u_e)$, $c(D) \neq c(Z) \neq c(A)$ if $u = v_B$, so $c(D) = c(A)$, and $c(D) \neq c(Z) = c(A)$ if $u \neq v_B$. This completes the induction and the proof of the claim.
\end{proof}

Let $(\Bcal, \Ical)$ be a solution to $c$.

\begin{claim}
	For every total Turing functional $\Phi_e$, there is an input $k$
	such that $\Ical \cap [k, \Phi_e(k)] = \emptyset$.
\end{claim}
\begin{proof}
By the padding lemma, we can assume that for all $A \in \Bcal$,
$A < e$. 
If $\Ical \cap [x_e, \Phi_e(x_e)] = \emptyset$ or $\Ical \cap [y_e, \Phi_e(y_e)] = \emptyset$, the we are done. Otherwise, let $S \subseteq X_e$ and $T \subseteq Y_e$ be such that $S, T \in \Ical$.
By assumption, $x_{e,s}, y_{e,s} > e$ for every $s \in \Nb$.
It follows that $A < e < S$. By the previous claim, $\Rcal_e$ is $(S,T)$-satisfied at some stage. Unfolding the definition, there is some $k > T$
such that $\Phi_e(k)\downarrow$ and for every $A < S$ (and in particular for every $A \in \Bcal$), either for every $B \subseteq [k, \Phi_e(k)]$, $c(A) \neq c(A \cup S \cup B)$,
or for every $B \subseteq [k, \Phi_e(k)]$, $c(A) \neq c(A \cup T \cup B)$.
In any case, $\Ical \cap [k, \Phi_e(k)] = \emptyset$. This completes the proof of the claim.
\end{proof}

As explained above, it follows that $\Ical$ is of hyperimmune-degree.
This completes the proof of Theorem~\ref{thm:lmfut-opt}.
\end{proof}

\begin{corollary}
$\rca + \wkl \nvdash \lmfut_2$
\end{corollary}
\begin{proof}
	By the relativized Hyperimmune-free Basis Theorem~\cite{Jockusch197201},
	this is a model of $\rca + \wkl$ with only hyperimmune-free degrees.
	By Theorem~\ref{thm:lmfut-opt}, this is not a model of $\lmfut_2$.
\end{proof}

Blass, Hirst and Simpson built a simple computable instance of the finite union theorem such that every solution computes the halting set: Given a finite set $S = \{x_0 < x_1 < \dots < x_n\}$, a gap $(x_i, x_{i+1})$ is \emph{large} if $\emptyset'\uh x_i = \emptyset'_{x_{i+1}} \uh x_i$,
	and is \emph{small} otherwise. A gap $(x_i, x_{i+1})$ is \emph{very small in $S$} if $\emptyset'_{x_n} \uh x_i \neq \emptyset'_{x_n} \uh x_{i+1}$.
	Letting $SG(S)$ and $VSG(G)$ denote the number of small gaps and of very small gaps in $S$, respectively, their coloring is simply defined by $c(S) = VSG(S) \mod 2$. Given an IP collection $\Ical$ homogeneous for $c$, they proved that $SG(S)$ is even for every $S \in \Ical$, and that the gap $(\max S, \min T)$ is large for every $S < T \in \Ical$. However, for this same instance, one can easily construct a computable full-match $(\Bcal, \Ical)$ with $|\Bcal| = 2$ as follows. Let $\Bcal = \{B_0, B_1\}$, where $SG(B_0) \mod 2 = SG(B_1) \mod 2 = 0$, $VSG(B_0)$ is odd, and $VSG(B_1)$ is even. Then $\Bcal$ full-matches $\Pcal_{fin}(\Nb) - \Bcal$. This motivates the following question.

\begin{question}
	Does $\lmfut_2$ or $\fmfut_2$ imply $\aca$ over $\rca$?
\end{question}

